FLEURS: Few-shot Learning Evaluation of Universal Representations of Speech

We introduce FLEURS, the Few-shot Learning Evaluation of Universal Representations of Speech benchmark. FLEURS is an n-way parallel speech dataset in 102 languages built on top of the machine translation FLoRes-101 benchmark, with approximately 12 hours of speech supervision per language. FLEURS can be used for a variety of speech tasks, including Automatic Speech Recognition (ASR), Speech Language Identification (Speech LangID), Translation and Retrieval. In this paper, we provide baselines for the tasks based on multilingual pre-trained models like mSLAM. The goal of FLEURS is to enable speech technology in more languages and catalyze research in low-resource speech understanding.

==> FLEURS (1)/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> FLEURS (1)/tables.tex <==
\newcommand{\insertcorpora}{
\begin{table*}[hbt!]
\scriptsize
\centering
\caption{Compare FLEURS to common public multilingual speech benchmarks.}
%We report per-language results for all geographical language groups. FLEURS is a dataset that is complete at more than 97\%. Some slight improvements and changes may be done in a 2nd version of the dataset (e.g. missing recordings, or replaced low-quality recordings). Updates will be made on our platform. We expect average results not to change significantly.}
\label{tab:corpora}

% 1
\begin{tabular}{l|cccccccc}
\toprule
% & \multicolumn{15}{c}{Western European}\\
% \midrule
Dataset &
\#Languages &
Total Duration &
Domains &
Speech Type &
Transcripts &
Parallel text &
Parallel speech &\\
\midrule
BABEL~\cite{gales2014babel} &
17 &
1k hours &
Conversational &
Spontaneous &
Yes &
No &
No & \\
CommonVoice~\cite{ardila2019common} &
93 &
15k hours &
Open domain &
Read &
Yes &
No &
No\\
CMU Wilderness~\cite{black2019cmu} &
700 &
14k hours &
Religion &
Read &
Yes &
Yes &
Yes\\
MLS~\cite{pratap2020mls} & 
8 &
50.5k hours &
Audiobook &
Read &
Yes &
No &
No & \\
CoVoST-2~\cite{wang2020covost2} &
22 &
2.9k hours &
Open domain &
Read &
Yes &
Yes &
No & \\
Voxlingua-107~\cite{valk2020voxlingua107} &
107 &
6.6k hours &
YouTube &
Spontaneous &
No &
No &
No\\
Europarl-ST~\cite{iranzo2020europarl} & 
6 &
500 hours &
Parliament &
Spontaneous &
Yes &
Yes &
No & \\
MuST-C~\cite{cattoni2021must} &
9 &
385 hours &
TED talks &
Spontaneous &
Yes &
Yes &
No & \\
mTEDx~\cite{salesky2021multilingual} & 
9 &
1k hours &
TED talks &
Spontaneous &
Yes &
Yes &
No & \\
VoxPopuli~\cite{wang2021voxpopuli} &
24 &
400k hours &
Parliament &
Spontaneous &
Partial &
Partial &
Partial & \\
CVSS~\cite{jia2022cvss} & 
22 &
1.1k hours &
Open domain &
Read/Synthetic &
Yes &
Yes &
Yes & \\
FLEURS (this work) & 
102 &
1.4k hours &
Wikipedia &
Read &
Yes &
Yes &
Yes\\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule
\bottomrule
\end{tabular}  
\caption{A comparison of commonly used datasets for multilingual speech representation learning, ASR, Speech Translation and Speech-LangID. CommonVoice statistics as on 24th May 2022.}
\end{table*}
}

% Region Group		Average train utterance duration in second	Average train utterance character number	Average test utterance duration in second	Average test utterance character number				
% Central-Asia/Middle-East/North-Africa (CMN)		12	104	13	108			
% CJK languages (CJK)		12	42	12	43				
% Eastern European (EE)		12	109	11	113				
% South Asian (SA)		12	106	12	110				
% South-East Asian (SEA)		14	119	14	123				
% Sub-Saharan African (SSA)		16	108	16	110				atern European (WE)		12	112	12	118
\newcommand{\insertfleursbasics}{
 \begin{table}[h!]
        \begin{center}
            \captionof{table}{Statistics for speech and transcript data in FLEURS.
            \label{tab:fleursbasics}}
            %\scriptsize
            \resizebox{\linewidth}{!}{
            \begin{tabular}[t]{l|ccccccc|c}
            \toprule
            % \multicolumn{3}{c}{\#hours for pre-training} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
            % \midrule
            {  Data Statistics} & WE & EE & CMN & SSA & SA & SEA & CJK & All \\
                \midrule
                % \multicolumn{1}{l|}{Number of languages} & 25 & 16 & 12 & 20 & 14 & 11 & 4 & 102 \\
                \midrule
                train speech hours & 231h & 134h & 116h & 237h & 124h & 112h & 32h & 987h \\
                dev speech hours & 29h & 18h & 14h & 24h & 16h & 14h & 4h & 120h \\
                test speech hours & 68h & 43h & 33h & 58h & 37h & 35h & 9h & 283h\\
                train transcript tokens & 1475k & 772k & 630k & 1072k & 699k & 525k & 405k & 5578k\\
                dev transcript tokens & 184k & 107k & 75k & 116k & 93k & 65k & 51k & 692k \\
                test transcript tokens & 443k & 260k & 181k & 272k & 210k & 158k & 116k & 1640k\\
                % \mctcb{2} & & & & & & & & \\
                \bottomrule
            \end{tabular}
            }
        \end{center}
    \end{table}
}

\newcommand{\insertFLEURS}{
\begin{table}[h!]
%\centering
\begin{tabular}{l|rrrrrr}
\toprule

ISO 639-3 & Language & Family & Subgrouping & Script & Bitext & Mono \\
afr & Afrikaans & Indo-European & Germanic & Latin & 570K & 26.1M \\
amh & Amharic & Afro-Asiatic & Afro-Asiatic & Ge’ez & 339K & 3.02M \\
ara & Arabic & Afro-Asiatic & Afro-Asiatic & Arabic & 25.2M & 126M \\
hye & Armenian & Indo-European & Other IE & Armenian & 977K & 25.4M \\
asm & Assamese & Indo-European & Indo-Aryan & Bengali & 43.7K & 738K \\
ast & Asturian & Indo-European & Romance & Latin & 124K & — \\
azj & Azerbaijani & Turkic & Turkic & Latin & 867K & 41.4M \\
bel & Belarusian & Indo-European & Balto-Slavic & Cyrillic & 42.4K & 24M \\
ben & Bengali & Indo-European & Indo-Aryan & Bengali & 2.16M & 57.9M \\
bos & Bosnian & Indo-European & Balto-Slavic & Latin & 187K & 15.9M \\
bul & Bulgarian & Indo-European & Balto-Slavic & Cyrillic & 10.3M & 235M \\
mya & Burmese & Sino-Tibetan & Sino-Tibetan+Kra-Dai & Myanmar & 283K & 2.66M \\
cat & Catalan & Indo-European & Romance & Latin & 5.77M & 77.7M \\
ceb & Cebuano & Austronesian & Austronesian & Latin & 484K & 4.11M \\
cmn & Mandarin Chinese & Sino-Tibetan & Sino-Tibetan+Kra-Dai & Han & 37.9M & 209M \\
yue & Cantonese Chinese & Sino-Tibetan & Sino-Tibetan+Kra-Dai & Han & 37.9M & 85.2M \\
hrv & Croatian & Indo-European & Balto-Slavic & Latin & 42.2K & 144M \\
ces & Czech & Indo-European & Balto-Slavic & Latin & 23.2M & 124M \\
dan & Danish & Indo-European & Germanic & Latin & 10.6M & 344M \\
nld & Dutch & Indo-European & Germanic & Latin & 82.4M & 230M \\
est & Estonian & Uralic & Uralic & Latin & 4.82M & 46M \\
tgl & Filipino (Tagalog) & Austronesian & Austronesian & Latin & 70.6K & 107M \\
fin & Finnish & Uralic & Uralic & Latin & 15.2M & 377M \\
fra & French & Indo-European & Romance & Latin & 289M & 428M \\
ful & Fula & Atlantic-Congo & Nilotic+Other AC & Latin & 71K & 531K \\
glg & Galician & Indo-European & Romance & Latin & 1.13M & 4.22M \\
lug & Ganda & Atlantic-Congo & Bantu & Latin & 14.4K & 537K \\
kat & Georgian & Kartvelian & Other & Georgian & 1.23M & 31.7M \\
deu & German & Indo-European & Germanic & Latin & 216M & 417M \\
ell & Greek & Indo-European & Other IE & Greek & 23.7M & 201M \\
guj & Gujarati & Indo-European & Indo-Aryan & Gujarati & 160K & 9.41M \\
hau & Hausa & Afro-Asiatic & Afro-Asiatic & Latin & 335K & 5.87M \\
heb & Hebrew & Afro-Asiatic & Afro-Asiatic & Hebrew & 6.64M & 208M \\
hin & Hindi & Indo-European & Indo-Aryan & Devanagari & 3.3M & 104M \\
hun & Hungarian & Uralic & Uralic & Latin & 16.3M & 385M \\
isl & Icelandic & Indo-European & Germanic & Latin & 1.17M & 37.5M \\
ibo & Igbo & Atlantic-Congo & Nilotic+Other AC & Latin & 145K & 693K \\
ind & Indonesian & Austronesian & Austronesian & Latin & 39.1M & 1.05B \\
gle & Irish & Indo-European & Other IE & Latin & 329K & 1.54M \\
ita & Italian & Indo-European & Romance & Latin & 116M & 179M \\
jpn & Japanese & Japonic & Other & Han, Hirgana, Katakana & 23.2M & 458M \\
jav & Javanese & Austronesian & Austronesian & Latin & 1.49M & 24.4M \\
kea & Kabuverdianu & Indo-European & Romance & Latin & 5.46K & 178K \\
kam & Kamba & Atlantic-Congo & Bantu & Latin & 50K & 181K \\
kan & Kannada & Dravidian & Dravidian & Telugu-Kannada & 155K & 13.1M \\
kaz & Kazakh & Turkic & Turkic & Cyrillic & 701K & 35.6M \\
khm & Khmer & Austro-Asiatic & Austro-Asiatic & Khmer & 398K & 8.87M \\
kor & Korean & Koreanic & Other & Hangul & 7.46M & 390M \\
kir & Kyrgyz & Turkic & Turkic & Cyrillic & 566K & 2.02M \\
lao & Lao & Kra-Dai & Sino-Tibetan+Kra-Dai & Lao & 153K & 2.47M \\
lav & Latvian & Indo-European & Balto-Slavic & Latin & 4.8M & 68.4M \\
lin & Lingala & Atlantic-Congo & Bantu & Latin & 21.1K & 336K \\
lit & Lithuanian & Indo-European & Balto-Slavic & Latin & 6.69M & 111M \\
luo & Luo & Nilo-Saharan & Nilotic+Other AC & Latin & 142K & 239K \\
ltz & Luxembourgish & Indo-European & Germanic & Latin & 3.41M & — \\
mkd & Macedonian & Indo-European & Balto-Slavic & Cyrillic & 1.13M & 28.8M \\
msa & Malay & Austronesian & Austronesian & Latin & 968K & 77.5M \\
mal & Malayalam & Dravidian & Dravidian & Malayalam & 497K & 24.8M \\
mlt & Maltese & Afro-Asiatic & Afro-Asiatic & Latin & 5.82M & — \\
mri & Maori & Austronesian & Austronesian & Latin & 196K & — \\
mar & Marathi & Indo-European & Indo-Aryan & Devanagari & 109K & 14.4M \\
mon & Mongolian & Mongolic & Other & Cyrillic & 555K & 20.4M \\
npi & Nepali & Indo-European & Indo-Aryan & Devanagari & 19.6K & 17.9M \\
nso & Northern Sotho & Atlantic-Congo & Bantu & Latin & 13.8K & 612K \\
nob & Norwegian & Indo-European & Germanic & Latin & 10.9M & 338M \\
nya & Nyanja & Atlantic-Congo & Bantu & Latin & 932K & — \\
oci & Occitan & Indo-European & Romance & Latin & 5.11K & — \\
ory & Oriya & Indo-European & Indo-Aryan & Oriya & 5K & 2.47M \\
orm & Oromo & Afro-Asiatic & Afro-Asiatic & Latin & 162K & 752K \\
pus & Pashto & Indo-European & Indo-Aryan & Perso-Arabic & 293K & 12M \\
fas & Persian & Indo-European & Indo-Aryan & Perso-Arabic & 6.63M & 611M \\
pol & Polish & Indo-European & Balto-Slavic & Latin & 40.9M & 256M \\
por & Portuguese (Brazil) & Indo-European & Romance & Latin & 137M & 340M \\
pan & Punjabi & Indo-European & Indo-Aryan & Gurmukhi & 142K & 5.02M \\
ron & Romanian & Indo-European & Romance & Latin & 31.9M & 391M \\
rus & Russian & Indo-European & Balto-Slavic & Cyrillic & 127M & 849M \\
srp & Serbian & Indo-European & Balto-Slavic & Cyrillic & 7.01M & 35.7M \\
sna & Shona & Atlantic-Congo & Bantu & Latin & 877K & — \\
snd & Sindhi & Indo-European & Indo-Aryan & Perso-Arabic & 21.8K & 314K \\
slk & Slovak & Indo-European & Balto-Slavic & Latin & 10.5M & 174M \\
slv & Slovenian & Indo-European & Balto-Slavic & Latin & 5.42M & 74.7M \\
som & Somali & Afro-Asiatic & Afro-Asiatic & Latin & 358K & 14.1M \\
ckb & Sorani Kurdish & Indo-European & Indo-Aryan & Arabic & 305K & 7.98M \\
spa & Spanish (Latin America) & Indo-European & Romance & Latin & 315M & 379M \\
swh & Swahili & Atlantic-Congo & Bantu & Latin & 349K & 35.8M \\
swe & Swedish & Indo-European & Germanic & Latin & 54.8M & 580M \\
tgk & Tajik & Indo-European & Indo-Aryan & Cyrillic & 544K & — \\
tam & Tamil & Dravidian & Dravidian & Tamil & 992K & 68.2M \\
tel & Telugu & Dravidian & Dravidian & Telugu-Kannada & 381K & 17.2M \\
tha & Thai & Kra-Dai & Sino-Tibetan+Kra-Dai & Thai & 10.6M & 319M \\
tur & Turkish & Turkic & Turkic & Latin & 41.2M & 128M \\
ukr & Ukrainian & Indo-European & Balto-Slavic & Cyrillic & 5.44M & 357M \\
umb & Umbundu & Atlantic-Congo & Bantu & Latin & 217K & 142K \\
urd & Urdu & Indo-European & Indo-Aryan & Perso-Arabic & 630K & 28M \\
uzb & Uzbek & Turkic & Turkic & Latin & — & 7.54M \\
vie & Vietnamese & Austro-Asiatic & Austro-Asiatic & Latin & 32.1M & 992M \\
cym & Welsh & Indo-European & Other IE & Latin & 826K & 12.7M \\
wol & Wolof & Atlantic-Congo & Nilotic+Other AC & Latin & 86.9K & 676K \\
xho & Xhosa & Atlantic-Congo & Bantu & Latin & 130K & 995K \\
yor & Yoruba & Atlantic-Congo & Nilotic+Other AC & Latin & 171K & 1.59M \\
zul & Zulu & Atlantic-Congo & Bantu & Latin & 123K & 994K \\
% \end{tabular}
\caption{101 languages in FLEURS statistics and table of results}
\label{tab:covost_enx_full}
% }
\end{table}
}


% \newcommand{\insertcorpora}{
% \begin{table*}[hbt!]
% \scriptsize
% \centering
% \caption{\textbf{  FLEURS full ASR results for all 102 languages}. }
% %We report per-language results for all geographical language groups. FLEURS is a dataset that is complete at more than 97\%. Some slight improvements and changes may be done in a 2nd version of the dataset (e.g. missing recordings, or replaced low-quality recordings). Updates will be made on our platform. We expect average results not to change significantly.}
% \label{tab:corpora}

% % 1
% \begin{tabular}{l|rrrrrrr}
% \toprule
% % & \multicolumn{15}{c}{Western European}\\
% % \midrule
% Language & ast & bs &  ca &  hr &  da &  nl \\
% %Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule 
% \midrule
% %\bottomrule
% \end{tabular}  

% \end{table*}
% }


\newcommand{\insertfleursfullasr}{
\begin{table*}[hbt!]
\scriptsize
\centering
\caption{FLEURS full ASR results, reporting \% CER ($\downarrow$), for all 102 languages.}
%We report per-language results for all geographical language groups. FLEURS is a dataset that is complete at more than 97\%. Some slight improvements and changes may be done in a 2nd version of the dataset (e.g. missing recordings, or replaced low-quality recordings). Updates will be made on our platform. We expect average results not to change significantly.}
\label{tab:fleurs_full}

% 1
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{15}{c}{Western European}\\
\midrule
Language & ast & bs &  ca &  hr &  da &  nl &  en &  fi &  fr &  gl &  de &  el &  hu &  is & ga \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
\wvbert & 8.7 & 5.8 & 4.3 & 9.3 & 11.3 & 6.0 & 17.2 & 3.0 & 9.6 & 8.6 & 8.0 & 11.7 & 24.9 & 11.9 & 39.5 \\
\mctcb{0.6} & 7.5 & 5.1 & 4.7 & 8.5 & 14.0 & 6.8 & 16.3 & 3.4 & 9.7 & 8.7 & 5.7 & 12.0 & 18.1 & 12.8 & 40.5 \\
%\bottomrule
\end{tabular}  

% 2
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{10}{c|}{Western European (WE)} & \multicolumn{5}{c}{Eastern European} \\
\midrule
Language & it &  kea &  lb &  mt &  nb &  oc &  pt &  es &  sv & cy & hy & be & bg & cs & et \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
\wvbert & 2.6 & 4.9 & 19.4 & 17.3 & 5.8 & 11.7 & 4.2 & 3.7 & 7.6 & 11.1 & 7.2 & 9.1 & 4.8 & 10.3 & 3.1 \\
\mctcb{0.6} & 2.3 & 5.1 & 21.0 & 17.3 & 6.1 & 12.7 & 4.4 & 3.3 & 7.8 & 12.0 & 7.8 & 7.5 & 5.2 & 9.2 & 3.5 \\
% \bottomrule
\end{tabular}  

% 3
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{11}{c|}{Eastern European (EE)} & \multicolumn{4}{c}{Central-Asia and}\\
\midrule
Language & ka & lv & lt & mk & pl & ro & ru & sr & sk & sl & uk & ar & az & he & kk \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
\wvbert & 30.7 & 4.4 & 12.8 & 11.8 & 5.0 & 8.0 & 5.6 & 11.6 & 4.9 & 7.9 & 21.4 & 10.5 & 12.7 & 37.2 & 6.5 \\
\mctcb{0.6} & 31.0 & 4.5 & 11.6 & 9.8 & 6.3 & 8.4 & 6.6 & 12.2 & 4.8 & 10.3 & 21.4 & 11.0 & 15.9 & 42.5 & 5.7 \\
% \bottomrule
\end{tabular}  

% 4
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{8}{c|}{Middle-East and North-Africa (CMN)} & \multicolumn{7}{c}{Sub-Saharan Africa}\\
\midrule
Language & ky & mn & ps & fa & ckb & tg & tr & uz & af & am & ff & lg & ha & ig & kam \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
\wvbert & 8.3 & 15.2 & 20.4 & 15.7 & 15.1 & 7.1 & 8.5 & 16.8 & 9.5 & 17.2 & 27.8 & 12.4 & 9.8 & 18.1 & 13.5 \\
\mctcb{0.6} & 8.0 & 16.1 & 21.1 & 10.0 & 15.0 & 7.6 & 9.7 & 15.5 & 11.9 & 17.8 & 27.5 & 12.9 & 10.5 & 18.7 & 14.0 \\
% \bottomrule
\end{tabular}  

% 5
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{13}{c|}{Sub-Saharan Africa (SSA)} & \multicolumn{2}{c}{South-Asia} \\
\midrule
Language & ln & luo & nso & ny & om & sn & so & sw & umb & wo & xh & yo & zu & as & bn \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
\wvbert & 6.1 & 7.0 & 11.7 & 11.5 & 21.7 & 16.6 & 21.3 & 19.4 & 13.1 & 17.8 & 23.9 & 23.3 & 9.8 & 13.7 & 9.4 \\
\mctcb{0.6} & 6.8 & 7.4 & 11.9 & 12.4 & 22.6 & 17.6 & 23.4 & 20.2 & 14.0 & 18.8 & 25.1 & 23.2 & 10.8 & 14.0 & 9.7 \\
% \bottomrule
\end{tabular}  

% 6
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{12}{c|}{South-Asia (SA)} & \multicolumn{3}{c}{South-East Asia}\\
\midrule
Language & gu & hi & kn & ml & mr & ne & or & pa & sd & ta & te & ur & my & ceb & fil\\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
\wvbert & 9.3 & 12.4 & 7.0 & 8.6 & 14.8 & 13.0 & 19.2 & 13.6 & 16.0 & 11.8 & 12.0 & 82.9 & 18.2 & 5.9 & 5.6 \\
\mctcb{0.6} & 9.6 & 15.2 & 9.6 & 12.2 & 18.9 & 14.8 & 20.7 & 15.2 & 20.8 & 13.2 & 12.3 & 83.1 & 18.8 & 6.2 & 5.5 \\
% \bottomrule
\end{tabular}  

% 7
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{8}{c|}{South-East Asia (SEA)} & \multicolumn{4}{c|}{CJK} & & & \\
\midrule
Language & id & jv & km & lo & ms & mi & th & vi & yue & cmn & ja & ko & All & & \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
\wvbert & 5.2 & 7.0 & 29.9 & 38.1 & 8.6 & 10.3 & 18.6 & 14.2 & 37.0 & 22.2 & 37.7 & 21.7 & 14.1 \\
\mctcb{0.6} & 5.6 & 7.1 & 30.2 & 37.5 & 7.2 & 11.2 & 20.1 & 14.3 & 39.8 & 23.1 & 39.2 & 22.4
 & 14.6 &  \\
\bottomrule
\end{tabular}  


\end{table*}
}



\newcommand{\insertfleursasr}{
 \begin{table*}[h!]
        \begin{center}
            \captionof{table}{\textbf{  Speech recognition }- Fleurs massively multilingual ASR baselines, reporting CER, by geographical group. Observe the discrepancy between European and African languages. {\color{blue} minm: as the benchmark, should we also report numbers on dev?}
            \label{tab:cer}}
            %\scriptsize
            \resizebox{0.8\linewidth}{!}{
            \begin{tabular}[t]{l|ccccccc|c}
            \toprule
            % \multicolumn{3}{c}{\#hours for pre-training} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
            % \midrule
            {  Model} & WE & EE & CMN & SSA & SA & SEA & CJK & All \\
                \midrule
                \multicolumn{1}{l|}{Number of languages} & 25 & 16 & 12 & 20 & 14 & 11 & 4 & 102 \\
                \midrule
                \wvbert & 11.6 & 9.9 & 16.4 & 23.6 & 20.0 & 18.7 & 34.5 & 17.0\\
                \mctcb{0.6} & 10.8 & 9.6 & 16.4 & 23.2 & 21.9 & 18.4 & 34.7 & 17.0 \\
                % \mctcb{2} & & & & & & & & \\
                \bottomrule
            \end{tabular}
            }
        \end{center}
    \end{table*}
}

% \newcommand{\insertfleursasrseenvsunseenwide}{
% \begin{table*}[h!]
%         \begin{center}
%     \begin{subtable}{0.5\textwidth}
%         \centering
%         \begin{tabular}{l|ccccccc|c}
%             \toprule
%             % \multicolumn{3}{c}{\#hours for pre-training} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
%             % \midrule
%             {  Groups} & WE & EE & CMN & SSA & SA & SEA & CJK & All \\
%                 \midrule
%                 \multicolumn{1}{l|}{Number of languages} & 17 & 11 & 7 & 3 & 7 & 5 & 2 & 52 \\
%                 \midrule
%                 \wvbert & 11.2 & 10.4 & 12.2 & 13.8 & 13.2 & 16.4 & 37.4& 13.1 \\
%                 \mctcb{2} & 11.0 & 10.7 & 11.7 & 14.6 & 14.3 & 16.7 & 39.5 & 13.3 \\
%                 \midrule
%                 %\wvbert & 10.5 & 9.1 & 12.2 & 14.7 & 14.5 & 18.2 & 37.2 & 13.0\\
%                 %\mctcb{0.6} & 11.6 & 9.9 & 13.5 & 15.6 & 16.2 & 19.1 & 40.3 & 14.2 \\
%                 % \mctcb{2} & & & & & & & & \\
%                 \bottomrule
%       \end{tabular}
%       \subcaption{Character error rate for seen languages}
%       \label{tab:seen}
%     \end{subtable}
%     \begin{subtable}{\textwidth}
%         \centering
%         \begin{tabular}{l|ccccccc|c}
%             \toprule
%             % \multicolumn{3}{c}{\#hours for pre-training} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
%             % \midrule
%             {  Groups} & WE & EE & CMN & SSA & SA & SEA & CJK & All \\
%                 \midrule
%                 \multicolumn{1}{l|}{Number of languages} & 8 & 11 & 7 & 17 & 7 & 6 & 2 & 50 \\
%                 \midrule
%                 \wvbert & 9.6 & 8.9 & 17.8 & 15.9 & 21.6 & 13.2 & 22.0 & 15.1 \\
%                 \mctcb{0.6} & 9.9 & 8.5 & 19.3 & 16.7 & 24.1 & 13.3 & 22.7 & 15.9\\
%                 % \wvbert & 9.7 & 9.0 & 17.6 & 15.3 & 22.0 & 15.3 & 22.1 & 15.8 \\
%                 % \mctcb{0.6} & 10.3 & 9.6 & 20.8 & 18.4 & 25.7 & 16.3 & 24.4 & 17.5 \\
%                 % \mctcb{2} & & & & & & & & \\
%                 \bottomrule
%         \end{tabular}
%         \subcaption{Character error rate for unseen languages}
%         \label{tab:unseen}
%      \end{subtable}
%     \begin{subtable}{\textwidth}
%         \centering
%         \begin{tabular}{l|ccccccc|c}
%             \toprule
%             % \multicolumn{3}{c}{\#hours for pre-training} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
%             % \midrule
%             {  Groups} & WE & EE & CMN & SSA & SA & SEA & CJK & All \\
%                 \midrule
%                 \multicolumn{1}{l|}{Number of languages} & 25 & 16 & 12 & 20 & 14 & 11 & 4 & 102 \\
%                 \midrule
%                 \wvbert  & 10.7 & 9.9 & 14.5 & 15.6 & 17.4 & 14.7 & 24.6 & 14.1 \\
%                 \mctcb{0.6} & 10.6 & 10.0 & 14.8 & 16.4 & 19.2 & 14.9 & 25.0 & 14.6 \\
%                 % \mctcb{2} & & & & & & & & \\
%                 \bottomrule
%         \end{tabular}
%         \subcaption{Character error rate for all languages}
%         \label{tab:unseen}
%      \end{subtable}
%      \caption{\textbf{  Speech recognition }- Fleurs massively multilingual ASR baselines, reporting CER, by geographical group. Observe the discrepancy between European and African languages}. % %{\color{blue} minm: as the benchmark, should we also report numbers on dev?}}
%      \label{tab:cer}
%              \end{center}
% \end{table*}
% }

% \newcommand{\insertsc}{
% \begin{table}[h!]
%         \begin{center}
%             \caption{{\bf Speech Classification }- Fleurs speech language identification accuracy. 
%             % {\color{blue} Let's update with the cleaned data, and show accuracy per region group?}
%             \label{tab:sc}}
%             % \scriptsize
%             \resizebox{0.9\linewidth}{!}{
%             \begin{tabular}{l|c}
%             \toprule
%                 {Model} & {Overall Accuracy}\\
%                 \midrule
%                 \wvbert & 71.4  \\
%                 \mctcb{0.6}  & 73.3 \\
%                 % \mctcb{2} & 77.7  \\
%                 \bottomrule
%             \end{tabular}
%             }
%       \vspace{-0.4cm}
%         \end{center}
%     \end{table}
% }

\newcommand{\insertsc}{
 \begin{table}[bht!]
        \begin{center}
            \captionof{table}{\textbf{  Speech identification }- FLEURS langID baselines, reporting \% accuracy ($\uparrow$), by geographical group.
            \label{tab:fleurssid}}
            %\scriptsize
            \resizebox{\linewidth}{!}{
            \begin{tabular}[t]{l|ccccccc|c}
            \toprule
            % \multicolumn{3}{c}{\#hours for pre-training} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
            % \midrule
            {  Model} & WE & EE & CMN & SSA & SA & SEA & CJK & Avg. \\
                \midrule
                \midrule
                \multicolumn{9}{l}{\it Speech identification accuracy for all languages} \\
                \midrule
                \multicolumn{1}{l|}{\# languages} & 25 & 16 & 12 & 20 & 14 & 11 & 4 & 102 \\
                \midrule
                \wvbert  & 85.3 & 78.4 & 72.9 & 59.1 & 52.0 & 65.7 & 89.7 & 71.4 \\
                
                \mctcb{0.6} & 84.6 & 81.3 & 75.9 & 62.2 & 51.7 & 73.4 & 87.8 & 73.3 \\
                % \midrule
                % \multicolumn{9}{l}{\it Speech identification accuracy for seen languages} \\
                % \midrule
                % \multicolumn{1}{l|}{Number of languages} & 17 & 11 & 7 & 3 & 7 & 5 & 2 & 52 \\
                % \midrule
                % \wvbert & 92.1\% & 87.2\% & 83.4\% & 61.1\% & 68.3\% & 82.5\% & 79.7\% & 84.3\% \\
                % \mctcb{2} & 92.8\% & 87.9\% & 86.1\% & 70.0\% & 68.0\% & 86.8\% & 72.0\% & 85.7\% \\
                % \midrule
                % \multicolumn{9}{l}{\it Speech identification accuracy for unseen languages} \\
                % \midrule
                % \multicolumn{1}{l|}{Number of languages} & 8 & 11 & 7 & 17 & 7 & 6 & 2 & 50 \\
                % \midrule                
                % \wvbert & 69.3\% & 59.1\% & 56.8\% & 58.8\% & 39.7\% & 55.4\% & 92.8\% & 58.5\% \\
                % \mctcb{0.6} & 65.4\% & 66.8\% & 60.4\% & 60.9\% & 39.5\% & 65.2\% & 92.5\% & 61.0\% \\
                % % \mctcb{2} & & & & & & & & \\
                \bottomrule
            \end{tabular}
            }
        \end{center}
    \end{table}
}

\newcommand{\insertfleursasrseenvsunseen}{
 \begin{table}[bht!]
        \begin{center}
            \captionof{table}{\textbf{  Speech recognition }- Fleurs massively multilingual ASR baselines, reporting \% CER ($\downarrow$), by geographical group.
            \label{tab:fleurs}}
            %\scriptsize
            \resizebox{\linewidth}{!}{
            \begin{tabular}[t]{l|ccccccc|c}
            \toprule
            % \multicolumn{3}{c}{\#hours for pre-training} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
            % \midrule
            {  Model} & WE & EE & CMN & SSA & SA & SEA & CJK & Avg. \\
                \midrule
                \midrule
                \multicolumn{9}{l}{\it Speech recognition CER for all languages} \\
                \midrule
                \multicolumn{1}{l|}{\# languages} & 25 & 16 & 12 & 20 & 14 & 11 & 4 & 102 \\
                \midrule
                \wvbert  & 10.7 & 9.9 & 14.5 & 15.6 & 17.4 & 14.7 & 24.6 & 14.1 \\
                \mctcb{0.6} & 10.6 & 10.0 & 14.8 & 16.4 & 19.2 & 14.9 & 25.0 & 14.6 \\
                % \midrule
                % \multicolumn{9}{l}{\it Speech recognition CER for seen languages} \\
                % \midrule
                % \multicolumn{1}{l|}{Number of languages} & 17 & 11 & 7 & 3 & 7 & 5 & 2 & 52 \\
                % \midrule
                % \wvbert & 11.2 & 10.4 & 12.2 & 13.8 & 13.2 & 16.4 & 37.4& 13.1 \\
                % \mctcb{2} & 11.0 & 10.7 & 11.7 & 14.6 & 14.3 & 16.7 & 39.5 & 13.3 \\
                % \midrule
                % \multicolumn{9}{l}{\it Speech recognition CER for unseen languages} \\
                % \midrule
                % \multicolumn{1}{l|}{Number of languages} & 8 & 11 & 7 & 17 & 7 & 6 & 2 & 50 \\
                % \midrule                
                % \wvbert & 9.6 & 8.9 & 17.8 & 15.9 & 21.6 & 13.2 & 22.0 & 15.1 \\
                % \mctcb{0.6} & 9.9 & 8.5 & 19.3 & 16.7 & 24.1 & 13.3 & 22.7 & 15.9\\
                % \mctcb{2} & & & & & & & & \\
                \bottomrule
            \end{tabular}
            }
        \end{center}
    \end{table}
}

\newcommand{\insertlanguages}{
\begin{table*}[ht!]
\begin{center}
% \scriptsize
\captionof{table}{\textbf{Characteristics of the 102 languages in FLEURS}, with their ISO codes, language families, estimated number of speakers in millions (\#S) from~\cite{Esch2022}.
Languages are grouped geographically in Western Europe (WE), Eastern Europe (EE), Central-Asia/Middle-East/North-Africa (CMN), Sub-Saharan Africa (SSA), South Asia (SA), South-East Asia (SEA) and CJK languages. Note that we make some minor changes compared to FLoRes, renaming ``Chinese (Simp)'' to ``Mandarin Chinese'' with code ``cmn'' (not ``zho'') and renaming ``Chinese (Trad)'' to ``Cantonese Chinese" with code ``yue'' (not ``zho''). 
\label{tab:langs}}
\begin{tabular}[t]{|r|l|l|l|l|l|r|}
\toprule
% \multicolumn{3}{c}{\#hours for pre-training} & 75 & 13 & 45 & \multicolumn{1}{l}{10h} & \\
% \midrule
Idx & Language & ISO 639-3 & ISO 639-1 & Family & Group & \#S \\ 
\midrule
1 & Afrikaans & afr & af & Indo-European & SSA & 17  \\ 
2 & Amharic & amh & am & Afro-Asiatic & SSA & 22  \\ 
3 & Arabic & ara & ar & Afro-Asiatic & CMN & 180  \\ 
4 & Armenian & hye & hy & Indo-European & EE & 6  \\ 
5 & Assamese & asm & as& Indo-European & SA & 13  \\ 
6 & Asturian & ast & - & Indo-European & WE & 0.6  \\ 
7 & Azerbaijani & azj & az & Turkic & CMN & 18  \\ 
8 & Belarusian & bel & be & Indo-European & EE & 3  \\ 
9 & Bengali & ben & bn & Indo-European & SA & 260  \\ 
10 & Bosnian & bos & bs& Indo-European & WE & 9  \\ 
11 & Bulgarian & bul & bg & Indo-European & EE & 7 \\ 
12 & Burmese & mya & my & Sino-Tibetan & SEA & 33  \\ 
13 & Cantonese Chinese & yue & - & Sino-Tibetan & CJK & 920  \\ 
14 & Catalan & cat & ca & Indo-European & WE & 4  \\ 
15 & Cebuano & ceb & - & Austronesian & SEA & 16  \\ 
16 & Croatian & hrv & hr & Indo-European & WE & 4  \\ 
17 & Czech & ces & cs & Indo-European & EE & 10  \\ 
18 & Danish & dan & da & Indo-European & WE & 5  \\ 
19 & Dutch & nld & nl & Indo-European & WE & 21  \\ 
20 & English & eng & en & Indo-European & WE & 550   \\
21 & Estonian & est & et & Uralic & EE & 1  \\ 
22 & Filipino (Tagalog) & tgl & tg & Austronesian & SEA & 22  \\ 
23 & Finnish & fin & fi & Uralic & WE & 5  \\ 
24 & French & fra & fr & Indo-European & WE & 280  \\ 
25 & Fula & ful & ff & Atlantic-Congo & SSA & 12  \\ 
26 & Galician & glg & gl & Indo-European & WE & 2  \\ 
27 & Ganda & lug & lg & Atlantic-Congo & SSA & 4  \\ 
28 & Georgian & kat & ka & Kartvelian & EE & 4  \\ 
29 & German & deu & de & Indo-European & WE & 83  \\ 
30 & Greek & ell & el &  Indo-European & WE & 13  \\ 
31 & Gujarati & guj & gu & Indo-European & SA & 56  \\ 
32 & Hausa & hau & ha &  Afro-Asiatic & SSA & 70  \\ 
33 & Hebrew & heb & he & Afro-Asiatic & CMN & 4  \\ 
34 & Hindi & hin & hi & Indo-European & SA & 320  \\ 
35 & Hungarian & hun & hu & Uralic & WE & 13  \\ 
36 & Icelandic & isl & is & Indo-European & WE &  0.3  \\ 
37 & Igbo & ibo & ig & Atlantic-Congo & SSA & 18  \\ 
38 & Indonesian & ind & id & Austronesian & SEA & 200  \\ 
39 & Irish & gle & ga & Indo-European & WE & 0.2  \\ 
40 & Italian & ita & it & Indo-European & WE & 61  \\ 
41 & Japanese & jpn & ja & Japonic & CJK & 130  \\ 
42 & Javanese & jav & jv & Austronesian & SEA & 85  \\ 
43 & Kabuverdianu & kea & - & Indo-European & WE & 0.9  \\ 
44 & Kamba & kam & - & Atlantic-Congo & SSA & 4  \\ 
45 & Kannada & kan & kn & Dravidian & SA & 43  \\ 
46 & Kazakh & kaz & kk & Turkic & CMN & 11  \\ 
47 & Khmer & khm & km & Austro-Asiatic & SEA & 16  \\ 
48 & Korean & kor & ko & Koreanic & CJK & 52  \\ 
49 & Kyrgyz & kir & ky & Turkic & CMN & 8  \\ 
50 & Lao & lao & lo & Kra-Dai & SEA & 20  \\ 
51 & Latvian & lav & lv & Indo-European & EE & 2  \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table*}
    

\begin{table*}[ht!]
\begin{center}
% \scriptsize
\begin{tabular}[t]{|r|l|l|l|l|l|r|}
\toprule
% \multicolumn{3}{c}{\#hours for pre-training} & 75 & 13 & 45 & \multicolumn{1}{l}{10h} & \\
% \midrule
Idx & Language & ISO 639-3 & ISO 639-1 & Family & Group & \#S \\ 
\midrule
52 & Lingala & lin & ln & Atlantic-Congo & SSA & 15   \\
53 & Lithuanian & lit & lt & Indo-European & EE & 2   \\
54 & Luo & luo & - & Nilo-Saharan & SSA & 4   \\
55 & Luxembourgish & ltz & lb & Indo-European & WE & 0.4   \\
56 & Macedonian & mkd & mk & Indo-European & EE & 1   \\
57 & Malay & msa & ms & Austronesian & SEA & 80   \\
58 & Malayalam & mal & ml & Dravidian & SA & 77   \\
59 & Maltese & mlt & mt & Afro-Asiatic & WE & 0.5   \\
60 & Mandarin Chinese & cmn & - & Sino-Tibetan & CJK & 80   \\
61 & Maori & mri & mi & Austronesian & SEA & 0.2   \\
62 & Marathi & mar & mr & Indo-European & SA & 83   \\
63 & Mongolian & mon & mn & Mongolic & CMN & 5   \\
64 & Nepali & npi & ne & Indo-European & SA & 16   \\
65 & Northern Sotho & nso & - & Atlantic-Congo & SSA & 14   \\
66 & Norwegian & nob & nb & Indo-European & WE & 5   \\
67 & Nyanja & nya & ny & Atlantic-Congo & SSA & 12   \\
68 & Occitan & oci & oc & Indo-European & WE & 0.5   \\
69 & Oriya & ory & or & Indo-European & SA & 35   \\
70 & Oromo & orm & om & Afro-Asiatic & SSA & 24   \\
71 & Pashto & pus & ps & Indo-European & CMN & 13   \\
72 & Persian & fas & fa & Indo-European & CMN & 40   \\
73 & Polish & pol & pl & Indo-European & EE & 38   \\
74 & Portuguese (Brazil) & por & pt & Indo-European & WE & 220   \\
75 & Punjabi & pan & pa & Indo-European & SA & 113   \\
76 & Romanian & ron & ro & Indo-European & EE & 19   \\
77 & Russian & rus & ru & Indo-European & EE & 150   \\
78 & Serbian & srp & sr & Indo-European & EE & 6   \\
79 & Shona & sna & sn & Atlantic-Congo & SSA & 9   \\
80 & Sindhi & snd & sd & Indo-European & SA & 68   \\
81 & Slovak & slk & sk & Indo-European & EE & 4   \\
82 & Slovenian & slv & sl & Indo-European & EE & 2   \\
83 & Somali & som & so & Afro-Asiatic & SSA & 24   \\
84 & Sorani Kurdish & ckb & - & Indo-European & CMN &  7   \\
85 & Spanish & spa & es & Indo-European & WE & 490   \\
86 & Swahili & swh & sw & Atlantic-Congo & SSA & 24   \\
87 & Swedish & swe & sv & Indo-European & WE & 8   \\
88 & Tajik & tgk & tg & Indo-European & CMN & 8   \\
89 & Tamil & tam & ta & Dravidian & SA & 76   \\
90 & Telugu & tel & te & Dravidian & SA & 82   \\
91 & Thai & tha & th & Kra-Dai & SEA & 20   \\
92 & Turkish & tur & tr & Turkic & CMN & 82   \\
93 & Ukrainian & ukr & uk & Indo-European & EE & 32   \\
94 & Umbundu & umb & - & Atlantic-Congo & SSA & 6   \\
95 & Urdu & urd & ur & Indo-European & SA & 120   \\
96 & Uzbek & uzb & uz & Turkic & CMN & 57   \\
97 & Vietnamese & vie & vi & Austro-Asiatic & SEA & 96   \\
98 & Welsh & cym & cy & Indo-European & WE & 0.7   \\
99 & Wolof & wol & wo & Atlantic-Congo & SSA & 4   \\
100 & Xhosa & xho & xh & Atlantic-Congo & SSA & 19   \\
101 & Yoruba & yor & yo & Atlantic-Congo & SSA & 21   \\
102 & Zulu & zul & zu & Atlantic-Congo & SSA & 11  \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table*}

}

% \newcommand{\insertfleursspeechtextretrieval}{
% \begin{table*}[hbt!]
% \scriptsize
% \centering
% \caption{\textbf{  FLEURS Speech-Text retrieval results for all 102 languages}. }
% %We report per-language results for all geographical language groups. FLEURS is a dataset that is complete at more than 97\%. Some slight improvements and changes may be done in a 2nd version of the dataset (e.g. missing recordings, or replaced low-quality recordings). Updates will be made on our platform. We expect average results not to change significantly.}
% \label{tab:fleurs_full}

% % 1
% \begin{tabular}{l|rrrrrrrrrrrrrrr}
% \toprule
% & \multicolumn{15}{c}{Western European}\\
% \midrule
% Language & ast & bs &  ca &  hr &  da &  nl &  en &  fi &  fr &  gl &  de &  el &  hu &  is & ga \\
% %Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule 
% \mctcb{0.6} & 90.1 & 95.5 & 93.2 & 98.0 & 94.1 & 95.3 & 96.0 & 93.0 & 90.7 & 90.9 & 91.2 & 81.2 & 85.3 & 71.7 & 55.1 \\
% %\bottomrule
% \end{tabular}  

% % 2
% \begin{tabular}{l|rrrrrrrrrrrrrrr}
% \toprule
% & \multicolumn{10}{c|}{Western European (WE)} & \multicolumn{5}{c}{Eastern European} \\
% \midrule
% Language & it &  kea &  lb &  mt &  nb &  oc &  pt &  es &  sv & cy & hy & be & bg & cs & et \\
% %Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule 
% \mctcb{0.6} & 93.5 & 95.4 & 80.5 & 92.7 & 91.9 & 77.4 & 91.9 & 69.6 & 94.2 & 82.3 & 50.3 & 90.2 & 95.1 & 98.1 & 95.6 \\
% % \bottomrule
% \end{tabular}  

% % 3
% \begin{tabular}{l|rrrrrrrrrrrrrrr}
% \toprule
% & \multicolumn{11}{c|}{Eastern European (EE)} & \multicolumn{4}{c}{Central-Asia and}\\
% \midrule
% Language & ka & lv & lt & mk & pl & ro & ru & sr & sk & sl & uk & ar & az & he & kk \\
% %Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule 
% \mctcb{0.6} & 70.5 & 97.4 & 96.8 & 96.1 & 95.8 & 92.0 & 93.2 & 97.7 & 97.6 & 97.4 & 93.5 & 82.7 & 83.0 & 64.0 & 88.7 \\
% % \bottomrule
% \end{tabular}  

% % 4
% \begin{tabular}{l|rrrrrrrrrrrrrrr}
% \toprule
% & \multicolumn{8}{c|}{Middle-East and North-Africa (CMN)} & \multicolumn{7}{c}{Sub-Saharan Africa}\\
% \midrule
% Language & ky & mn & ps & fa & ckb & tg & tr & uz & af & am & ff & lg & ha & ig & kam \\
% %Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule 
% \mctcb{0.6} & 84.3 & 70.7 & 84.8 & 85.4 & 80.8 & 76.3 & 84.5 & 67.6 & 90.1 & 34.1 & 81.4 & 90.7 & 84.5 & 85.8 & 89.7 \\
% % \bottomrule
% \end{tabular}  

% % 5
% \begin{tabular}{l|rrrrrrrrrrrrrrr}
% \toprule
% & \multicolumn{13}{c|}{Sub-Saharan Africa (SSA)} & \multicolumn{2}{c}{South-Asia} \\
% \midrule
% Language & ln & luo & nso & ny & om & sn & so & sw & umb & wo & xh & yo & zu & as & bn \\
% %Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule 
% \mctcb{0.6} & 91.2 & 91.0 & 80.8 & 85.5 & 92.7 & 84.1 & 68.7 & 91.2 & 77.3 & 90.6 & 90.9 & 92.4 & 85.5 & 81.5 & 83.5 \\
% % \bottomrule
% \end{tabular}  

% % 6
% \begin{tabular}{l|rrrrrrrrrrrrrrr}
% \toprule
% & \multicolumn{12}{c|}{South-Asia (SA)} & \multicolumn{3}{c}{South-East Asia}\\
% \midrule
% Language & gu & hi & kn & ml & mr & ne & or & pa & sd & ta & te & ur & my & ceb & tg\\
% %Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule 
% \mctcb{0.6} & 77.0 & 78.0 & 69.0 & 62.3 & 69.8 & 66.1 & 15.7 & 70.6 & 71.8 & 58.0 & 73.5 & 70.6 & 2.4 & 79.8 & 76.3 \\
% % \bottomrule
% \end{tabular}  

% % 7
% \begin{tabular}{l|rrrrrrrrrrrrrrr}
% \toprule
% & \multicolumn{8}{c|}{South-East Asia (SEA)} & \multicolumn{4}{c|}{CJK} & & & \\
% \midrule
% Language & id & jv & km & lo & ms & mi & th & vi & yue & cmn & ja & ko & All & & \\
% %Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
% \midrule 
% \mctcb{0.6} & 79.6 & 78.0 & 42.1 & 37.0 & 77.7 & 64.7 & 3.2 & 64.5 & 5.4 & 2.4 & 5.8 & 5.2
%  & 76.9 &  \\
% \bottomrule
% \end{tabular}  


% \end{table*}
% }

\newcommand{\insertfleursspeechtextretrieval}{
\begin{table*}[hbt!]
\scriptsize
\centering
\caption{FLEURS Speech-to-Text and Text-to-Speech retrieval results, reporting \% P@1 ($\uparrow$), for all 102 languages. }
%We report per-language results for all geographical language groups. FLEURS is a dataset that is complete at more than 97\%. Some slight improvements and changes may be done in a 2nd version of the dataset (e.g. missing recordings, or replaced low-quality recordings). Updates will be made on our platform. We expect average results not to change significantly.}
\label{tab:fleurs_full_retrieval}

% 1
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{15}{c}{Western European}\\
\midrule
Language & ast & bs &  ca &  hr &  da &  nl &  en &  fi &  fr &  gl &  de &  el &  hu &  is & ga \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
Speech-to-Text Retrieval & 90.1 & 95.5 & 93.2 & 98.0 & 94.1 & 95.3 & 96.0 & 93.0 & 90.7 & 90.9 & 91.2 & 81.2 & 85.3 & 71.7 & 55.1 \\
Text-to-Speech Retrieval & 83.5 & 95.1 & 87.0 & 95.3 & 90.1 & 87.1 & 94.4 & 90.6 & 80.6 & 81.0 & 81.9 & 74.6 & 88.4 & 67.4 & 56.7 \\

%\bottomrule
\end{tabular}  

% 2
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{10}{c|}{Western European (WE)} & \multicolumn{5}{c}{Eastern European} \\
\midrule
Language & it &  kea &  lb &  mt &  nb &  oc &  pt &  es &  sv & cy & hy & be & bg & cs & et \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
Speech-to-Text Retrieval & 93.5 & 95.4 & 80.5 & 92.7 & 91.9 & 77.4 & 91.9 & 69.6 & 94.2 & 82.3 & 50.3 & 90.2 & 95.1 & 98.1 & 95.6 \\
Text-to-Speech Retrieval & 86.0 & 95.6 & 78.8 & 89.0 & 85.7 & 85.2 & 88.9 & 61.5 & 90.4 & 79.6 & 52.5 & 85.5 & 92.1 & 96.3 & 94.1 \\
% \bottomrule
\end{tabular}  

% 3
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{11}{c|}{Eastern European (EE)} & \multicolumn{4}{c}{Central-Asia and}\\
\midrule
Language & ka & lv & lt & mk & pl & ro & ru & sr & sk & sl & uk & ar & az & he & kk \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
Speech-to-Text Retrieval & 70.5 & 97.4 & 96.8 & 96.1 & 95.8 & 92.0 & 93.2 & 97.7 & 97.6 & 97.4 & 93.5 & 82.7 & 83.0 & 64.0 & 88.7 \\
Text-to-Speech Retrieval & 66.9 & 95.7 & 94.0 & 92.7 & 92.0 & 86.4 & 89.2 & 95.6 & 95.6 & 94.8 & 88.9 & 82.7 & 75.2 & 71.3 & 89.7 \\

% \bottomrule
\end{tabular}  

% 4
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{8}{c|}{Middle-East and North-Africa (CMN)} & \multicolumn{7}{c}{Sub-Saharan Africa}\\
\midrule
Language & ky & mn & ps & fa & ckb & tg & tr & uz & af & am & ff & lg & ha & ig & kam \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
Speech-to-Text Retrieval & 84.3 & 70.7 & 84.8 & 85.4 & 80.8 & 76.3 & 84.5 & 67.6 & 90.1 & 34.1 & 81.4 & 90.7 & 84.5 & 85.8 & 89.7 \\
Text-to-Speech Retrieval & 78.6 & 70.4 & 78.7 & 85.5 & 76.9 & 70.7 & 81.0 & 63.5 & 86.7 & 40.3 & 65.8 & 90.6 & 85.8 & 90.2 & 90.7 \\
% \bottomrule
\end{tabular}  

% 5
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{13}{c|}{Sub-Saharan Africa (SSA)} & \multicolumn{2}{c}{South-Asia} \\
\midrule
Language & ln & luo & nso & ny & om & sn & so & sw & umb & wo & xh & yo & zu & as & bn \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
Speech-to-Text Retrieval & 91.2 & 91.0 & 80.8 & 85.5 & 92.7 & 84.1 & 68.7 & 91.2 & 77.3 & 90.6 & 90.9 & 92.4 & 85.5 & 81.5 & 83.5 \\
Text-to-Speech Retrieval & 95.2 & 88.3 & 83.4 & 84.9 & 90.2 & 79.1 & 69.0 & 91.2 & 83.6 & 90.8 & 88.9 & 90.7 & 84.2 & 78.8 & 77.6 \\

% \bottomrule
\end{tabular}  

% 6
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{12}{c|}{South-Asia (SA)} & \multicolumn{3}{c}{South-East Asia}\\
\midrule
Language & gu & hi & kn & ml & mr & ne & or & pa & sd & ta & te & ur & my & ceb & fil \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
Speech-to-Text Retrieval & 77.0 & 78.0 & 69.0 & 62.3 & 69.8 & 66.1 & 15.7 & 70.6 & 71.8 & 58.0 & 73.5 & 70.6 & 2.4 & 79.8 & 73.1 \\
Text-to-Speech Retrieval & 73.6 & 66.0 & 67.1 & 57.1 & 70.0 & 62.4 & 18.6 & 70.2 & 64.1 & 54.5 & 67.2 & 33.1 & 2.6 & 75.6 & 69.5 \\

% \bottomrule
\end{tabular}  

% 7
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
& \multicolumn{8}{c|}{South-East Asia (SEA)} & \multicolumn{4}{c|}{CJK} & & & \\
\midrule
Language & id & jv & km & lo & ms & mi & th & vi & yue & cmn & ja & ko & All & & \\
%Train Hours & 264h & 184h & 113h & 136h & 49h & 44h & 18h & 10h & 10h & 4h & 2h & 3h \\
\midrule 
Speech-to-Text Retrieval & 79.6 & 78.0 & 42.1 & 37.0 & 77.7 & 64.7 & 3.2 & 64.5 & 2.4 & 5.4 & 5.8 & 5.2 & 76.9 &  \\
Text-to-Speech Retrieval & 75.3 & 72.5 & 49.3 & 47.7 & 73.7 & 74.8 & 3.8 & 64.4 & 2.7 & 5.1 & 8.3 & 2.9 & 74.4 & \\
\bottomrule
\end{tabular}  


\end{table*}
}


\newcommand{\insertretrievalseenvsunseen}{
 \begin{table}[bht!]
        \begin{center}
            \captionof{table}{\textbf{  Cross-modal Speech-Text Retrieval }- FLEURS massively multilingual Speech-to-Text and Text-to-Speech retrieval baselines, reporting \% P@1 ($\uparrow$) score, by geographical group.
            \label{tab:fleurs_retrieval}}
            %\scriptsize
            \resizebox{\linewidth}{!}{
            \begin{tabular}[t]{l|ccccccc|c}
            \toprule
            % \multicolumn{3}{c}{\#hours for pre-training} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
            % \midrule
            {Task} & WE & EE & CMN & SSA & SA & SEA & CJK & Avg. \\
                \midrule
                \midrule
                \multicolumn{9}{l}{\it P@1 for all languages} \\
                \midrule
                \multicolumn{1}{l|}{\# languages} & 25 & 16 & 12 & 20 & 14 & 11 & 4 & 102 \\
                \midrule
                Speech-to-Text Retrieval & 87.6 & 91.1 & 79.4 & 83.9 & 67.7 & 54.8 & 4.7 & 76.9 \\
                Text-to-Speech Retrieval & 83.7 & 88.3 & 77.1 & 83.5 & 61.4 & 55.4 & 4.7 & 74.4 \\
                % \midrule
                % \multicolumn{9}{l}{\it P@1 for seen languages} \\
                % \midrule
                % \multicolumn{1}{l|}{Number of languages} & 17 & 11 & 7 & 3 & 7 & 5 & 2 & 52 \\
                % \midrule
                % Speech-to-Text Retrieval & 88.1 & 93.4 & 83.0 & 89.1 & 62.1 & 52.9 & 5.6 & 78.9 \\
                % Text-to-Speech Retrieval & 83.7 & 90.3 & 81.0 & 88.7 & 58.3 & 53.3 & 6.7 & 76.1 \\
                % \midrule
                % \multicolumn{9}{l}{\it P@1 for unseen languages} \\
                % \midrule
                % \multicolumn{1}{l|}{Number of languages} & 8 & 11 & 7 & 17 & 7 & 6 & 2 & 50 \\
                % \midrule                
                % Speech-to-Text Retrieval & 86.6 & 86.0 & 74.4 & 83.0 & 71.8 & 56.3 & 3.8 & 75.0 \\
                % Text-to-Speech Retrieval & 84.0 & 83.7 & 71.5 & 82.5 & 63.8 & 57.1 & 2.8 & 72.7 \\
                % \mctcb{2} & & & & & & & & \\
                \bottomrule
            \end{tabular}
            }
        \end{center}
    \end{table}
}



\newcommand{\insertspeechtextretrievalhparams}{
\begin{table}[ht]
  \centering
  \begin{tabular}{lr}
    \toprule
    Hyperparameter & Value \\
    \midrule
    Batch size & $128$ utt.\\
    LR schedule & Linear warm-up and decay \\
    Warmup Ratio & $0.2$ \\
    Peak learning rate & $2e^{-4}$ \\
    Number of Epochs & $20$ \\
    Adam eps  & $1e^{-9}$ \\
    Adam betas  & ($0.9$, $0.999$)\\
    Weight decay & $1e^{-6}$ \\
    \bottomrule
  \end{tabular}
  \caption{Hyperparameters for Speech-Text Retrieval Task.}
  \label{tab:hp-pretrain-asr}
\end{table}
}

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


